Simpler Context-Dependent Logical Forms via Model Projections

We consider the task of learning a context-dependent mapping from utterances to denotations. With only denotations at training time, we must search over a combinatorially large space of logical forms, which is even larger with context-dependent utterances. To cope with this challenge, we perform successive projections of the full model onto simpler models that operate over equivalence classes of logical forms. Though less expressive, we find that these simpler models are much faster and can be surprisingly effective. Moreover, they can be used to bootstrap the full model. Finally, we collected three new context-dependent semantic parsing datasets, and develop a new left-to-right parser.

==> sfig/bin/mpto1pdf <==
#!/bin/bash

# Converts a Metapost file <prefix>.mp into a PDF file <prefix>.pdf.
# If -quiet is set, writes to <prefix>.log.
# Uses a <prefix>.tmp directory (doesn't delete if conversion failed).
#
# This is a wrapper for mptopdf, and is a messy hack, but then again, mptopdf
# is kind of messy.
#
# Percy Liang
# 08/24/07
#
# This script is taken from rfig with a few modifications.
# Updated 04/20/13

if [ $# -lt 1 ]; then
  echo "Usage: `basename $0` [-quiet] <metapost file>"
  exit 1
fi

bindir=`dirname $0`
if [[ $bindir != /* ]]; then
  bindir=$PWD/$bindir
fi

if [ "$1" == "-quiet" ]; then
  quiet=1
  shift
else
  quiet=0
fi
p=$1; p=${p/\.mp/} # Prefix
tmp=$p.tmp
rm -rf $tmp || exit 1

# Make sure after the end of the run, the pdf file (whether it got created or
# not) corresponds to the mp file.
rm -f $p.pdf || exit 1

if [ $quiet == 1 ]; then
  out=../`basename $p`.log
else
  out=/dev/stdout
fi

# Hack: copy fmt file to the right place.
mkdir -p $HOME/.texmf-var/web2c || exit 1
cp $bindir/mptopdf.fmt $HOME/.texmf-var/web2c || exit 1

mkdir $tmp || exit 1 # Create temporary directory
(
  cd $tmp || exit 1
  echo "mpto1pdf: writing to $tmp" > $out || exit 1

  p=`basename $p`
  # Link up the files so it looks like we are running in that current directory
  for x in ../*; do
    ln -sf $x || exit 1
  done
  # Do not symlink the old file or the log
  rm -f $p.pdf $p-*.pdf $p.log || exit 1

  # Convert to pdf files
  # Stupid mptopdf does not return exit code 1 if it fails
  # But ls $p-*.pdf should fail
  if [ $quiet == 1 ]; then
    $bindir/mptopdf -metafun $p.mp < /dev/null >> $out 2>&1 || (echo ==================================================; cat $out $p.tmp/mpxerr.log; exit 1)
  else
    $bindir/mptopdf -metafun $p.mp || exit 1
  fi

  # Join pdf files
  $bindir/pdfjoin --outfile $p.pdf \
    `/bin/ls $p-*.pdf 2>/dev/null | awk -F '-' '{print $NF,$0}' | sort -n | awk '{print $2}'` >> $out 2>&1 || exit 1

  cp $p.pdf .. || exit 1
  echo "Output written successfully to $p.pdf" >> $out || exit 1
) || exit 1
rm -r $tmp || exit 1 # Remove temporary directory


==> sfig/bin/mptopdf <==
eval '(exit $?0)' && eval 'exec perl -S $0 ${1+"$@"}' && eval 'exec perl -S $0 $argv:q'
        if 0;

# MikTeX users can set environment variable TEXSYSTEM to "miktex".

#D \module
#D   [       file=mptopdf.pl,
#D        version=2010.05.28, %  2000.05.29
#D          title=converting MP to PDF,
#D       subtitle=\MPTOPDF,
#D         author=Hans Hagen,
#D           date=\currentdate,
#D            url=www.pragma-ade.nl,
#D      copyright={PRAGMA ADE / Hans Hagen \& Ton Otten}]
#C
#C This module is part of the \CONTEXT\ macro||package and is
#C therefore copyrighted by \PRAGMA. See licen-en.pdf for
#C details.

# use File::Copy ; # not in every perl

use Config ;
use Getopt::Long ;
use strict ;
use File::Basename ;

$Getopt::Long::passthrough = 1 ; # no error message
$Getopt::Long::autoabbrev  = 1 ; # partial switch accepted

my $Help    = 0 ;
my $Latex   = 0 ;
my $TeXexec = 0 ;
my $RawMP   = 1 ;
my $MetaFun = 0 ;
my $PassOn  = '' ;

&GetOptions
  ( "help"    => \$Help  ,
    "rawmp"   => \$RawMP, # option is now default, but keep for compat
    "metafun" => \$MetaFun,
    "passon"  => \$PassOn, # option is ignored, but keep for compat
    "latex"   => \$Latex,
    "texexec" => \$TeXexec) ;

my $program       = "MPtoPDF 1.4.1" ;
my $pattern       = "@ARGV" ; # was $ARGV[0]
my $miktex        = 0 ;
my $done          = 0 ;
my $report        = '' ;
my $mplatexswitch = " --tex=latex " ;
my $texexecswitch = " --tex=\"texexec --batch --once --nomp --mptex\" " ; # untested

my $dosish      = ($Config{'osname'} =~ /^(ms)?dos|^os\/2|^mswin/i) ;
my $escapeshell = (($ENV{'SHELL'}) && ($ENV{'SHELL'} =~ m/sh/i ));

if ($ENV{"TEXSYSTEM"}) {
    $miktex = ($ENV{"TEXSYSTEM"} =~ /miktex/io) ;
}

my @files ;
my $command = my $mpbin = ''  ;

# agressive copy, works for open files like in gs

sub CopyFile {
    my ($From,$To) = @_ ;
    return unless open(INP,"<$From") ;
    return unless open(OUT,">$To") ;
    binmode INP ;
    binmode OUT ;
    while (<INP>) {
        print OUT $_ ;
    }
    close (INP) ;
    close (OUT) ;
}

if (($pattern eq '')||($Help)) {
    print "\n$program : provide MP output file (or pattern)\n" ;
    exit ;
} elsif ($pattern =~ /\.mp$/io) {
    shift @ARGV ; my $rest = join(" ", @ARGV) ;
    if (open(INP,$pattern)) {
        while (<INP>) {
            if (/(documentstyle|documentclass|begin\{document\})/io) {
                $Latex = 1 ; last ;
            }
        }
        close (INP) ;
    }
    if ($Latex) {
      $rest .= " $mplatexswitch" ;
    }
    if ($TeXexec) {
      $rest .= " $texexecswitch" ;
    }
    if ($MetaFun) {
      $mpbin = "mpost --progname=mpost --mem=metafun" ;
    } else {
      $mpbin = "mpost --mem=mpost" ;
    }
    my $runner = "$mpbin $rest $pattern" ;
    print "\n$program : running '$runner'\n" ;
    my $error =  system ($runner) ;
    if ($error) {
        print "\n$program : error while processing mp file\n" ;
        exit 1 ;
    } else {
        $pattern =~ s/\.mp$//io ;
        @files = glob "$pattern.*" ;
    }
} elsif (-e $pattern) {
    @files = ($pattern) ;
} elsif ($pattern =~ /.\../o) {
    @files = glob "$pattern" ;
} else {
    $pattern .= '.*' ;
    @files = glob "$pattern" ;
}

foreach my $file (@files) {
    $_ = $file ;
    if (s/\.(\d+|mps)$// && -e $file) {
        if ($miktex) {
            $command = "pdftex -undump=mptopdf" ;
        } else {
            $command = "pdftex -fmt=mptopdf -progname=context" ;
        }
        if ($dosish) {
            $command = "$command \\relax $file" ;
        } else {
            $command = "$command \\\\relax $file" ;
        }
        my $error = system($command) ;
        if ($error) {
            print "\n$program : error while processing tex file\n" ;
            exit 1 ;
        }
        my $pdfsrc = basename($_).".pdf";
        rename ($pdfsrc, "$_-$1.pdf") ;
        if (-e $pdfsrc) {
            CopyFile ($pdfsrc, "$_-$1.pdf") ;
        }
        if ($done) {
            $report .= " +" ;
        }
        $report .= " $_-$1.pdf" ;
        ++$done  ;
    }
}

if ($report eq '') {
    $report = '*' ;
}

if ($done) {
    print "\n$program : $pattern is converted to$report\n" ;
} else {
    print "\n$program : no filename matches $pattern\n" ;
}


==> sfig/create-presentation <==
#!/bin/bash

if [ $# != 1 ]; then
  echo "Usage: `basename $0` <directory to create presentation>"
  exit 1
fi

out=$1

mkdir -p $out || exit 1

# Link to this directory
abspath () { case "$1" in /*)printf "%s\n" "$1";; *)printf "%s\n" "$PWD/$1";; esac; }
real=`abspath $(dirname $0)`
ln -sf $real $out/sfig || exit 1

cat <<EOF > $out/index.html 
<head>
  <script src="sfig/internal/sfig.js"></script>
  <script src="sfig/internal/Graph.js"></script>
  <script src="sfig/internal/RootedTree.js"></script>
  <script src="sfig/internal/seedrandom.js"></script>
  <script src="utils.js"></script>
  <script src="index.js"></script>
</head>
<body onload="prez.run()">
</body>
EOF

cat <<EOF > $out/utils.js
G = sfig.serverSide ? global : this;
sfig.importAllMethods(G);

// Latex macros
sfig.latexMacro('R', 0, '\\\\mathbb{R}');
sfig.latexMacro('P', 0, '\\\\mathbb{P}');
sfig.latexMacro('E', 0, '\\\\mathbb{E}');
sfig.latexMacro('diag', 0, '\\\\text{diag}');

sfig.initialize();

G.prez = sfig.presentation();

// Useful functions (not standard enough to put into an sfig library).

G.frameBox = function(a) { return frame(a).bg.strokeWidth(1).fillColor('white').end; }
G.bigFrameBox = function(a) { return frameBox(a).padding(10).scale(1.4); }

G.bigArrow = function(a, b) { return arrow(a, b).strokeWidth(10).color('brown'); }
G.bigLeftArrow = function(s) { return leftArrow(s || 100).strokeWidth(10).color('brown'); }
G.bigRightArrow = function(s) { return rightArrow(s || 100).strokeWidth(10).color('brown'); }
G.bigUpArrow = function(s) { return upArrow(s || 100).strokeWidth(10).color('brown'); }
G.bigDownArrow = function(s) { return downArrow(s || 100).strokeWidth(10).color('brown'); }

G.xseq = function() { return new sfig.Table([arguments]).center().margin(5); }
G.yseq = function() { return ytable.apply(null, arguments).margin(10); }

G.stmt = function(prefix, suffix) {
  var m;
  if (!suffix && (m = prefix.match(/^([^:]+): (.+)$/))) {
    prefix = m[1];
    suffix = m[2];
  }
  return prefix.fontcolor('darkblue') + ':' + (suffix ? ' '+suffix : '');
}
G.headerList = function(title) {
  var contents = Array.prototype.slice.call(arguments).slice(1);
  return ytable.apply(null, [title ? stmt(title) : _].concat(contents.map(function(line) {
    if (line == _) return _;
    if (typeof(line) == 'string') return bulletedText([null, line]);
    if (line instanceof sfig.PropertyChanger) return line;
    return indent(line);
  })));
}

G.node = function(x, shaded) { return overlay(circle(20).fillColor(shaded ? 'lightgray' : 'white') , x).center(); }
G.indent = function(x, n) { return frame(x).xpadding(n != null ? n : 20).xpivot(1); }
G.stagger = function(b1, b2) { b1 = std(b1); b2 = std(b2); return overlay(b1.numLevels(1), pause(), b2); }

G.dividerSlide = function(text) {
  return slide(null, nil(), parentCenter(text)).titleHeight(0);
}

G.moveLeftOf = function(a, b, offset) { return transform(a).pivot(1, 0).shift(b.left().sub(offset == null ? 5 : offset), b.ymiddle()); }
G.moveRightOf = function(a, b, offset) { return transform(a).pivot(-1, 0).shift(b.right().add(offset == null ? 5 : offset), b.ymiddle()); }
G.moveTopOf = function(a, b, offset) { return transform(a).pivot(0, 1).shift(b.xmiddle(), b.top().up(offset == null ? 5 : offset)); }
G.moveBottomOf = function(a, b, offset) { return transform(a).pivot(0, -1).shift(b.xmiddle(), b.bottom().down(offset == null ? 5 : offset)); }
G.moveCenterOf = function(a, b) { return transform(a).pivot(0, 0).shift(b.xmiddle(), b.ymiddle()); }
EOF

cat <<EOF > $out/index.js
// For node.js
require('./sfig/internal/sfig.js');
require('./sfig/internal/Graph.js');
require('./sfig/internal/RootedTree.js');
require('./sfig/internal/metapost.js');
require('./sfig/internal/seedrandom.js');
require('./utils.js');

// Title slide
prez.addSlide(slide(nil(),
  ytable('(title)', '(subtitle)').center().scale(1.3).strokeColor('darkblue'),
  ytable(
    text('(your name)').scale(1.2),
  _).center().ymargin(20),
  ytable(
    nowrapText('(venue)'),
    'June 7, 2013',
  _).center().scale(0.8),
_).body.center().end.showIndex(false).showHelp(true));

// First introduction slide
prez.addSlide(slide('Introduction',
  stmt('Goal', 'write a presentation'),
  pause(),
  headerList('Points',
    'first',
    'second',
    'third',
  _),
  pause(),
  parentCenter(
    xseq(frameBox('problem'), bigRightArrow(), frameBox('solution')).center(),
  _),
_));

prez.addSlide(dividerSlide('To be continued...'.italics()));

// For node.js: output PDF (you must have Metapost installed).
prez.writePdf({outPrefix: 'index'});
EOF

echo "Your presentation has been created in $out."
echo "To view it, point your browser to: $out/index.html"
echo "To edit it, open: $out/index.js"
echo "To generate PDF (via node.js and Metapost), type: (cd $out && node index.js)"

